A Simple Non-Deterministic Approach Can Adapt to Complex Unpredictable 5G Cellular Networks

5G cellular networks are envisioned to support a wide range of emerging delay-oriented services with different delay requirements (e.g., 20ms for VR/AR, 40ms for cloud gaming, and 100ms for immersive video streaming). However, due to the highly variable and unpredictable nature of 5G access links, existing end-to-end (e2e) congestion control (CC) schemes perform poorly for them. In this paper, we demonstrate that properly blending non-deterministic exploration techniques with straightforward proactive and reactive measures is sufficient to design a simple yet effective e2e CC scheme for 5G networks that can: (1) achieve high controllable performance, and (2) possess provable properties. To that end, we designed Reminis and through extensive experiments on emulated and real-world 5G networks, show the performance benefits of it compared with different CC schemes. For instance, averaged over 60 different 5G cellular links on the Standalone (SA) scenarios, compared with a recent design by Google (BBR2), Reminis can achieve 2.2x lower 95th percentile delay while having the same link utilization.

==> Evaluation/FA_figs.tex <==
\begin{figure}
    \centering
    \includesvg[width=0.85\linewidth]{Evaluation/figures/AIMD.svg}
    \caption{Role of AIMD Module}
    \label{AIMD}
\end{figure}
% \begin{figure}
%     \centering
    
%     \begin{subfigure}[b]{0.48\linewidth}        %% or \columnwidth
%         \centering
%          \includesvg[width=\linewidth]{Evaluation/figures/AIMD.svg}
%         \caption{Role of AIMD Module}
%         \label{AIMD}
       

%     \end{subfigure}
%     \begin{subfigure}[b]{0.48\linewidth}        %% or \columnwidth
%         \centering
%          \includesvg[width=\linewidth]{Evaluation/figures/NDE_final.svg}
%         \caption{Role of NDE Module}
%         \label{NDE}
       

%     \end{subfigure}

% \begin{subfigure}[b]{0.48\linewidth}        %% or \columnwidth
%         \centering
%          \includesvg[width=\linewidth]{Evaluation/figures/new_CM.svg}
%         \caption{Role of CM Module}
%         \label{CM}
       

%     \end{subfigure}
%     \begin{subfigure}[b]{0.48\linewidth}        %% or \columnwidth
%         \centering
%          \includesvg[width=\linewidth]{Evaluation/figures/new_PS.svg}
%          \caption{Role of PS Module}
%         \label{PS}
       

%     \end{subfigure}


    
%     \caption{Reminis and 5G Challenges}
%     \label{step}
% \end{figure}

==> Evaluation/deepdive_figs2.tex <==
\begin{figure} [h]
    \centering
    \begin{subfigure}[b]{0.48\linewidth}        %% or \columnwidth
        \centering
          \includegraphics[width=0.95\linewidth]{Evaluation/figures/fairness.pdf}
         \caption{Reminis Fairness}
        \label{fairness}

    \end{subfigure}
    \begin{subfigure}[b]{0.48\linewidth}        %% or \columnwidth
        \centering
       \includegraphics[width=0.95\linewidth]{Evaluation/figures/cpu_util.pdf}
         \caption{Avg. CPU Utilization}
        \label{cpu_util}

    \end{subfigure}


    \caption{Reminis Fairness and CPU Utilization}
    \label{util_fair}
\end{figure}





==> ack.tex <==
\section*{Acknowledgments}


==> analysis.tex <==
\section{Analysis}

